Asynchronous and Parallel Distributed Pose Graph Optimization

We present Asynchronous Stochastic Parallel Pose Graph Optimization (ASAPP), the first asynchronous algorithm for distributed pose graph optimization (PGO) in multi-robot simultaneous localization and mapping. By enabling robots to optimize their local trajectory estimates without synchronization, ASAPP offers resiliency against communication delays and alleviates the need to wait for stragglers in the network. Furthermore, ASAPP can be applied on the rank-restricted relaxations of PGO, a crucial class of non-convex Riemannian optimization problems that underlies recent breakthroughs on globally optimal PGO. Under bounded delay, we establish the global first-order convergence of ASAPP using a sufficiently small stepsize. The derived stepsize depends on the worst-case delay and inherent problem sparsity, and furthermore matches known result for synchronous algorithms when there is no delay. Numerical evaluations on simulated and real-world datasets demonstrate favorable performance compared to state-of-the-art synchronous approach, and show ASAPP's resilience against a wide range of delays in practice.

==> introduction_v2.tex <==


Simultaneous localization and mapping (SLAM) involves the joint determination of the position of an autonomous platform within its environment (localization) and the determination of attributes of its domain of operation such the presence of (or properties of) obstacles (mapping). SLAM is a fundamental capability in GPS-denied environments, but robustness concerns and acquisition latency arise when all information is gathered by a single device. Multi-robot SLAM alleviates these issues, and avoids the ambiguities of stitching distinct maps together through the definition of a common pose graph. For this reason, \emph{pose graph optimization} (PGO) is the backbone of state of the art approaches to multi-robot SLAM. To date, however, approaches to this problem require synchronous processing of observations at a base station. The goal of this work is to develop decentralized asynchronous PGO, which mitigates communication, privacy, and vulnerability concerns associated with centralization.

In PGO, we seek to estimate all robots' trajectories from noisy relative pose measurements, which amounts to search over the special orthogonal group, i.e., rotation matrices, for the one that minimizes the quadratic error between the rotation and translation of one robot observed by another, summed over all robots. Riemannian optimization, i.e., projected gradient methods whose gradients are computed in terms of Riemannian metrics, has been proposed to address these problems in the centralized case \cite{RosenSESyncIJRR19,Briales2017RAL,Tian2019RBCD}. Moreover, the development of distributed algorithms for PGO has gained attention recently \cite{Choudhary2017Distributed,Lajoie2019RAL,Tian2019RBCD}. 

To the best of our knowledge, however, existing distributed PGO algorithms are inherently \emph{synchronous}, which necessitates that robots, for instance, pass messages over the network or wait at predetermined points, in order to ensure up-to-date information during optimization. Doing so may incur considerable communication overhead and increases the complexity of implementation. On the other hand, dropping synchronization in the execution of synchronous algorithms may cause divergence, both in theory and practice.


%\subsection{Distributed and Parallel PGO}

In pursuit of decentralized asynchronous algorithms for convergent PGO, we note that synchronized decentralized Riemannian optimization has been well-studied -- see \cite{Tron2009CDC,Tron2012Thesis,Tron2014,Tron2016} for consensus protocol approaches. The key insight which departs from vanilla distributed gradient method \cite{bertsekas1989parallel} is the definition of a set of reshaped cost functions based on the geodesic distance. These insights, have been combined with, e.g., line-search \cite{Knuth2012ICRA}, or augmented Lagrangians \cite{Choudhary2015IROS}, or two-stage relaxation schemes \cite{Choudhary2017Distributed}. The two-stage relaxation approach has further led to the development of outlier rejection schemes \cite{Lajoie2019RAL}. One challenge with the aforementioned works is that the non-convex constraint implies Lagrangian relaxations will have positive duality gap, and successive approximations may converge to a poor stationary point. To ameliorate this issue, semi-definite relaxations have gained traction. Specifically, in related work \cite{Tian2019RBCD}, we avoid Lagrangian relaxation by directly optimizing PGO and its rank-restricted semidefinite relaxations (see \cite{Briales2017RAL}) using Riemannian gradients. In a separate line of research, \cite{Fan2019ISRR} propose an accelerated PGO solver suitable for distributed settings based on generalized proximal operators. 

The aforementioned works are promising, but critically rely on \emph{synchronization} that limits their practical value for networked autonomous systems. However, we note that there is a plethora of works attempting to parallelize optimization algorithms and execute  updates without synchrony. Sufficient conditions for the convergence of asynchronous gradient-based methods began with \cite{bertsekas1989parallel}, and have since been used to develop asynchronous randomized block coordinate and stochastic gradient algorithms -- see \cite{Agarwal2011NIPS,Niu2011NIPS,Liu2015SIAM,Liu2015JMLR,Lian2018ICML} and references therein. We are especially interested in asynchronous parallel schemes for non-convex optimization, which have been studied in \cite{Lian2015NIPS,Cannelli2019}. In this work, we generalize these approaches to the setting where the feasible set is a the product of Riemannian manifolds, motivated by PGO.
Our model of asynchrony is comparable to \cite{Lian2018ICML}: workers exchange local models asynchronously during optimization. 
However, unlike \cite{Lian2018ICML}, we obviate the need for local averaging to achieve consensus, as each robot is only responsible for updating its own trajectory.  


%
%% Cunningham et al. \cite{CunninghamDDFSAM,CunninghamDDFSAM2} propose a distributed algorithm for feature-based SLAM in which robots exchange condensed graphs after applying linearization and Gaussian elimination.  
%%Choudhary et al. \cite{Choudhary2015IROS} proposes the alternating direction method of multipliers (ADMM) as a decentralized method to solve PGO.  
%However, convergence of ADMM is not established due to the non-convex nature of the optimization problem. 
%More recently, Choudhary et al. \cite{Choudhary2017Distributed} propose a two-stage approach that first uses distributed successive over-relaxation (SOR) \cite{bertsekas1989parallel} to solve the underlying rotation synchronization problem after chordal relaxation.
%In the second stage, SOR is used again to solve a single Gauss-Newton iteration over the full problem. 
%This approach is also adopted by Lajoie et al.~\cite{Lajoie2019RAL}, and the authors further implement distributed outlier rejection during PGO.
%In our recent work \cite{Tian2019RBCD}, we avoid explicit linearization by directly optimizing PGO and its rank-restricted semidefinite relaxations \cite{Briales2017RAL}. 
%The proposed solver performs distributed block-coordinate descent over the product of Riemannian manifolds, and provably converge to first-order critical points with global sublinear rate. 
%In a separate line of research, Fan and Murphey~\cite{Fan2019ISRR} propose an accelerated PGO solver suitable for distributed optimization based on generalized proximal methods. 




%While the aforementioned works show promising progress, all of them critically rely on the \emph{synchronization} assumption that limits their practical value in the distributed setting. 
%Specifically, the need for local processes to wait and synchronize over the network (e.g., to receive the most up-to-date messages from others) often result in unnecessary latency in the system and substantially increase the difficulty of implementation. 
%In this work, we overcome this important challenge by developing the first \emph{asynchronous} and provably \emph{delay-tolerant} algorithm for distributed PGO and provide the associated convergence analysis.


%\subsection{Asynchronous Parallel Optimization}
%
%In recent years, parallel and asynchronous optimization algorithms have received tremendous attention due to popular applications such as large-scale machine learning and deep learning.
%Early studies of asynchronous optimization include the seminal work of Bertsekas and Tsitsiklis \cite{bertsekas1989parallel}, who establish
%sufficient conditions for the convergence of asynchronous gradient-based methods. 
%Later works such as \cite{Agarwal2011NIPS,Niu2011NIPS,Liu2015SIAM,Liu2015JMLR,Lian2015NIPS,Cannelli2019,Lian2018ICML} develop a family of asynchronous algorithms (e.g., based on stochastic gradient descent or randomized coordinate descent) and providing explicit convergence rate estimates. 
%Some works, including \cite{Lian2015NIPS,Cannelli2019}, specifically consider asynchronous algorithms for \emph{non-convex} optimization. 
%In this paper, we draw inspirations from these prior work and develop an asynchronous algorithm on the product of Riemannian manifolds to solve PGO.
%Our model is similar to the decentralized asynchronous model of Lian et al. \cite{Lian2018ICML}, in which workers exchange local models asynchronously during optimization. 
%However, unlike \cite{Lian2018ICML}, our method avoids averaging local models to achieve consensus, since each robot is only responsible for updating its own trajectory.  


{\bf \noindent Contributions} The result, then, is a new method for PGO called $\ALGORITHM$ (\textbf{A}synchronous \textbf{S}toch\textbf{A}stic \textbf{P}arallel \textbf{P}ose \textbf{G}raph \textbf{O}ptimization) the first \emph{asynchronous} algorithm for distributed PGO. Further, we establish this method converges to a first-order critical point for a sufficiently small step-size  and under suitable hypotheses of the (at-worst bounded) delay due to asynchrony. The step-size selection depends on the maximum delay and inherent problem sparsity.
%
%We take inspiration from parallel and asynchronous algorithms in Euclidean optimization \cite{bertsekas1989parallel,Agarwal2011NIPS,Niu2011NIPS,Liu2015SIAM,Lian2015NIPS}, and adapt these ideas to solve the non-convex Riemannian optimization problem underlying PGO.
%In $\ALGORITHM$, each robot executes its local optimization loop without waiting for others. Doing so makes $\ALGORITHM$ easier to implement in practice and flexible against communication delay, where local optimization processes can run at a much faster rate compared to synchronous algorithms. 
Furthermore, we show that the same algorithm can be applied straightforwardly to solve the so-called rank-restricted semidefinite relaxations of PGO, a crucial class of non-convex Riemannian optimization problems that lies at the heart of recent global PGO solvers \cite{RosenSESyncIJRR19,Briales2017RAL,Tian2019RBCD}.
%
%Since asynchronous algorithms allow communication delays to be substantial and unpredictable, it is generally expected that conditions for their convergence are more stringent compared to their synchronous counterparts.
%In this work, we provide a rigorous convergence analysis for $\ALGORITHM$.
%We show that as long as the delay is not arbitrarily large, $\ALGORITHM$ always converges to first-order critical points using a sufficiently small stepsize. 
Numerical evaluations on simulated and real-world datasets demonstrate the effectiveness of $\ALGORITHM$ in reducing the delay due to communications latency, which improves the practicality of distributed PGO.%, and also verify its resilience against delay during distributed optimization. 



%
%
%
%\subsection*{Contributions}
%We present $\ALGORITHM$,
%the first \emph{asynchronous} and \emph{parallel} algorithm for solving Riemannian optimization problems underlying distributed pose graph optimization and its rank-restricted semidefinite relaxations. 
%$\ALGORITHM$ is provably \emph{delay-tolerant}:
%under bounded delay, we prove that the algorithm converges to first-order critical points using a sufficiently small stepsize that varies as a function of maximum delay and problem sparsity. 
%We further demonstrate the effectiveness of $\ALGORITHM$ on both simulated and real-world SLAM datasets, and show its resilience against communication delay.

==> problem.tex <==

% \begin{figure}
% 	\centering
% 	\begin{tikzpicture}[scale=1.5]
% 	\tikzstyle{special vertex}=[circle,draw,very thick,color=red]
% 	\node[special vertex] at (0.85,2.598076) (v1) {};
% 	\node[special vertex] at (2.15,2.598076) (v2) {};
% 	\node[special vertex] at (2.75,1.499037) (v3) {};
% 	\node[special vertex] at (2.15, 0.433013) (v4) {};
% 	\node[special vertex] at (0.85, 0.433013) (v5) {};
% 	\node[special vertex] at (0.25,1.499037) (v6) {};
% 	%%%%%%%
% 	\node (c1) at (0.95,2.90) [] {$x_{_1}$};
% 	\node (c2) at (2.25,2.90) [] {$x_{_2}$};
% 	\node (c4) at (3.05,1.25) [] {$x_{_3}$};
% 	\node (c6) at (2.25,0.10) [] {$x_{_4}$};
% 	\node (c5) at (0.95,0.10) [] {$x_{_5}$};
% 	\node (c3) at (0.10,1.25) [] {$x_{_6}$};
% 	%%%%%%%
% 	\draw[](v1) -- (v2);
% 	\draw[](v2) -- (v3);
% 	\draw[](v3) -- (v4);
% 	\draw[](v4) -- (v5);
% 	\draw[](v5) -- (v6);
% 	\draw[](v6) -- (v1);
% 	%
% 	\draw[](v2) -- (v4);
% 	\draw[](v2) -- (v6);
% 	\draw[](v4) -- (v6);
% 	%%%%%%%
% 	\end{tikzpicture}
% 	\caption{\small Example pose graph. \todo{more...} }
% 	\label{fig:pose_graph_example}
% \end{figure} 


\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.24\textwidth}
		\centering
		\begin{tikzpicture}[scale=1.1]
		\tikzstyle{vertex}=[circle,fill,scale=0.4,draw]
		\tikzstyle{special vertex}=[circle,fill=gray!30,scale=0.4,draw]
		\tikzstyle{square vertex}=[rectangle,fill,scale=0.5,draw]
		\tikzstyle{diamond vertex}=[regular polygon,regular polygon
		sides=3,rotate=45,fill,scale=0.3,draw]
		\node[special vertex] at (1,   2.5) (a1) {};
		\node[vertex] at (1.5, 2.5) (a2) {};
		\node[special vertex] at (2,   2.5) (a3) {};
		
		\node[special vertex] at (0.5, 2.0) (b1) {};
		\node[vertex] at (0.5, 1.5) (b2) {};
		\node[special vertex] at (0.5, 1.0) (b3) {};
		
		\node[vertex] at (2.5, 2.0) (c1) {};
		\node[special vertex] at (2.5, 1.5) (c2) {};
		\node[vertex] at (2.5, 1.0) (c3) {};
		
		\node[vertex] at (1,   0.5) (d1) {};
		\node[special vertex] at (1.5, 0.5) (d2) {};
		\node[vertex] at (2,   0.5) (d3) {};
		%%%%%%%
		\node (r1) at (1.5,3.0) [] {\faAndroid$_{_1}$};
		\node (r2) at (0.15,  1.5) [] {\faAndroid$_{_2}$};
		\node (r3) at (2.90, 1.5) [] {\faAndroid$_{_3}$};
		\node (r4) at (1.5, 0) [] {\faAndroid$_{_4}$};
		%%%%%%%
		\draw[](a1) -- (a2);
		\draw[](a2) -- (a3);
		\draw[](b1) -- (b2);
		\draw[](b2) -- (b3);
		\draw[](c1) -- (c2);
		\draw[](c2) -- (c3);
		\draw[](d1) -- (d2);
		\draw[](d2) -- (d3);
		
		\draw[](a2) -- (b2);
		\draw[](a2) -- (c1);
		\draw[](c1) -- (d3);
		\draw[](a2) -- (c3);
		\draw[](b2) -- (d1);
		\draw[](b2) -- (d3);
		\begin{pgfonlayer}{background}
			\node[fit=(a1)(a2)(a3),rounded corners,fill=violet!15,inner xsep=3pt,inner ysep=4pt] {};
			\node[fit=(b1)(b2)(b3),rounded corners,fill=green!15,inner xsep=3pt,inner ysep=4pt] {};
			\node[fit=(c1)(c2)(c3),rounded corners,fill=cyan!15,inner xsep=3pt,inner ysep=4pt] {};
			\node[fit=(d1)(d2)(d3),rounded corners,fill=orange!15,inner xsep=3pt,inner ysep=4pt] {};
		\end{pgfonlayer}
		\end{tikzpicture}
		\captionsetup{justification=centering}
		\caption{\small Pose graph $G$}
		\label{fig:pose_graph}
	\end{subfigure}
	~
	\begin{subfigure}[t]{0.20\textwidth}
		\centering
		\begin{tikzpicture}[scale=0.8]
		\tikzstyle{vertex}=[circle,scale=1,draw]
		%%%%%%%
		\node[vertex,fill=violet!15] at (1.5,3.0) (r1) {$x_1$};
		\node[vertex,fill=green!15]  at (0.15,  1.5) (r2) {$x_2$};
		\node[vertex,fill=cyan!15] at (2.90, 1.5) (r3) {$x_3$};
		\node[vertex,fill=orange!15]  at (1.5, 0)  (r4) {$x_4$};
		%%%%%%%
		\draw[thick] (r1) -- (r2);
		\draw[thick] (r1) -- (r3);
		\draw[thick] (r2) -- (r4);
		\draw[thick] (r3) -- (r4);
		%%%%%%%
		\end{tikzpicture}
		\captionsetup{justification=centering}
		\caption{\small Robot-level graph $G_{\Rcal}$}
		\label{fig:robot_graph}
	\end{subfigure}
	\caption
	{\small 
	(a) Example pose graph $G$ with $4$ robots, each with $3$ poses. 
	Each edge denotes a relative pose measurement (edge direction is omitted).
	Private poses are colored in gray. 
	(b) Corresponding robot-level graph $G_{\Rcal}$. 
	Two robots are connected if they share any relative measurements (inter-robot loop closures). 
	Note that for robot $i$ to optimize its pose estimates $x_i$, it only needs to receive its neighboring poses through the network.
	At any time, robot $i$ does not need to know the private poses of any other robots.
  	}
	\label{fig:example_graph}
\end{figure}



In this section, we formally define pose graph optimization (PGO) in the context of multi-robot SLAM. 
Given relative pose measurements (possibly between different robots), we aim to \emph{jointly} estimate the trajectories of all robots in a common reference frame.
Let $\Rcal = \{1, 2, \hdots, n\}$ be the set of robots. 
Denote the pose of robot $i \in \Rcal$ at time step $\tau$ as $T_{i_\tau} = (R_{i_\tau}, t_{i_\tau}) \in \SE(d)$, where $d \in \{2,3\}$ is the dimension of the estimation problem.
A relative pose measurement from $T_{i_\tau}$ to $T_{j_s}$ is denoted as 
$\widetilde{T}^{i_\tau}_{j_s} = (\widetilde{R}^{i_\tau}_{j_s}, \widetilde{t}^{i_\tau}_{j_s}) \in \SE(d)$. 
Following \cite{RosenSESyncIJRR19,Briales2017RAL,Tian2019RBCD}, we assume the following generative noise model for our measurements, 
\begin{align}
    \widetilde{R}^{i_\tau}_{j_s} &= \underline{R}^{i_\tau}_{j_s} R^{\epsilon},   &&{R}^{\epsilon} \sim \Langevin(I_d, w_R),
    \label{eq:rotation_noise_model} \\
    \widetilde{t}^{i_\tau}_{j_s} &= \underline{t}^{i_\tau}_{j_s} + t^{\epsilon}, && {t}^{\epsilon} \sim \Ncal(0, w_t^{-1} I_d).
    \label{eq:translation_noise_model}
\end{align}
Above, $\Langevin(I_d, w_R)$ is the isotropic Langevin distribution with concentration parameter $w_R$ \cite{RosenSESyncIJRR19}, and $\underline{T}^{i_\tau}_{j_s} = (\underline{R}^{i_\tau}_{j_s}, \underline{t}^{i_\tau}_{j_s}) \in \SE(d)$ denotes the ground truth (i.e., noiseless) relative transformation. For notation convenience, in \eqref{eq:rotation_noise_model} and \eqref{eq:translation_noise_model} we have assumed the same noise parameters for all relative measurements. Our approach trivially generalizes to the case where measurements have different noise parameters, which is the standard setup in prior work \cite{Tian2019RBCD,RosenSESyncIJRR19,Briales2017RAL}.
It can be shown that maximum likelihood estimation (MLE) corresponds to solving the following {non-convex} optimization problem,
\begin{problem}[Maximum Likelihood Estimation]
	\normalfont
	\begin{subequations}
		\begin{align}
		& \underset{}{\text{min}}
		\sum_{(i_\tau,j_s) \in E} w_R \norm{R_{j_s} - R_{i_{\tau}} \widetilde{R}^{i_{\tau}}_{j_s}}_\text{F}^2 
		+ w_t \norm{t_{j_s} - t_{i_{\tau}} - R_{i_{\tau}} \widetilde{t}^{i_{\tau}}_{j_s}}^2_2, \nonumber \\
		& \text{s.t.} \;\;\;
		R_{i_{\tau}} \in \SOd(d), \; t_{i_{\tau}} \in \mathbb{R}^d, \; \forall i \in \Rcal, \; \forall \tau.
		\label{eq:mle}
		\tag{$\text{P}_1$}
		\end{align}
	\end{subequations}
	\label{prob:mle}
\end{problem}
\vspace{-0.5cm}

Problem~\eqref{eq:mle} can be compactly represented with a \emph{pose graph} $G \triangleq (V, E)$, where each vertex in $V$ corresponds to a single pose owned by a robot. 
We add a directed edge from $i_{\tau}$ to $j_s$ to $E$ if and only if there is a relative measurement from $T_{i_{\tau}}$ to $T_{j_s}$. 
Figure~\ref{fig:pose_graph} shows an example pose graph.

In this paper, we also consider the so-called \emph{rank-restricted semidefinite relaxation} of \eqref{eq:mle} \cite{RosenSESyncIJRR19}. 
Define the Stiefel manifold as $\Stiefel(d,r) \triangleq \{Y \in \mathbb{R}^{r \times d}: Y^\top T = I_d\}$, where $r \geq d$. 
The rank-$r$ relaxation of \eqref{eq:mle} is defined as the following non-convex Riemannian optimization problem,
\begin{problem}[Rank-$r$-restricted Semidefinite Relaxation]
	\normalfont
	\begin{subequations}
		\begin{align}
		& \underset{}{\text{min}}
		\sum_{(i_{\tau},j_s) \in E} w_R \norm{Y_{j_s} - Y_{i_{\tau}} \widetilde{R}^{i_{\tau}}_{j_s}}_\text{F}^2 
		+ w_t \norm{p_{j_s} - p_{i_{\tau}} - Y_{i_{\tau}} \widetilde{t}^{i_{\tau}}_{j_s}}^2_2, \nonumber \\
		& \text{s.t.} \;\;\;
		Y_{i_{\tau}} \in \Stiefel(d,r), \; p_{i_{\tau}} \in \mathbb{R}^r, \; \forall i \in \Rcal, \; \forall \tau.
		\tag{$\text{P}_2$}
		\label{eq:qcqp}
		\end{align}
	\end{subequations}
	\label{prob:qcqp}
\end{problem}
\vspace{-0.5cm}

With $r = d$, we have $\Stiefel(d,d) = \Orthogonal(d)$ and \eqref{eq:qcqp} is also known as the \emph{orthogonal relaxation} of \eqref{eq:mle}, obtained by dropping the determinant constraint on $\SOd(d)$.
As $r$ increases beyond $d$, we obtain a hierarchy of rank-restricted problems, each having the form of \eqref{eq:qcqp} but with a slightly ``lifted'' search space as determined by $r$.
This hierarchy of rank-restricted problems lies at the heart of the so-called Riemannian Staircase procedure \cite{Boumal2015BlockDiagonal} for solving the semidefinite relaxation of \eqref{eq:mle}, which has proven extremely successful in the design of global solvers for PGO \cite{RosenSESyncIJRR19, Briales2017RAL, Tian2019RBCD}.
% We refer the reader to \cite{RosenSESyncIJRR19,Tian2019RBCD,Boumal2016NIPS} for in-depth discussions on the favorable theoretical properties enjoyed by \eqref{eq:qcqp} and the semidefinite relaxation. 
Once we solve \eqref{eq:qcqp} either globally or locally to a critical point, we can apply a distributed \emph{rounding} procedure (e.g. as detailed in \cite{Tian2019RBCD}) to obtain an feasible solution to the original MLE problem \eqref{eq:mle}.
Furthermore, note that \eqref{eq:qcqp} shares the same sparsity structure as encoded by the pose graph.

For the purpose of designing a distributed optimization algorithm (Section~\ref{sec:algorithm}), it is more convenient to represent \eqref{eq:mle} and \eqref{eq:qcqp} as the following optimization problem defined on the level of robots,
\begin{problem}[Robot-level Optimization Problem]
	\normalfont
	\begin{equation}
		\begin{aligned}
		& \underset{}{\text{min}}
		\sum_{(i,j) \in E_R} f_{ij}(x_i, x_j) + \sum_{i \in \Rcal} h_i(x_i),  \\
		& \text{s.t.} \;\;\;
		x_i \in \Mcal_i, \; \forall i \in \Rcal.
		\end{aligned}
		\tag{$\text{P}$}
		\label{eq:P}
	\end{equation}
	\label{prob:P}
\end{problem}
\vspace{-0.5cm}

In \eqref{eq:P}, each variable $x_i$ concatenates all variables owned by robot $i \in \Rcal$. 
For instance, for \eqref{eq:qcqp}, $x_i$ contains all the ``lifted'' rotation  and translation variables of robot $i$. 
Let $n_i$ be the number of poses of robot $i$.
Then,
\begin{align}
    x_i &= \begin{bmatrix}
    Y_{i_1} & p_{i_1} & \hdots & Y_{i_{n_i}} & p_{i_{n_i}}
    \end{bmatrix}, \\
    \Mcal_i &= (\Stiefel(d,r) \times \mathbb{R}^r)^{n_i}.
\end{align}

The cost function in \eqref{eq:P} consists of a set of \emph{shared costs} $f_{ij}: \Mcal_i \times \Mcal_j \to \mathbb{R}$ between pairs of robots, and a set of \emph{private costs} $h_i: \Mcal_i \to \mathbb{R}$ for individual robots.  
For both \eqref{eq:mle} and \eqref{eq:qcqp}, $f_{ij}$ is formed by relative measurements between any of robot $i$'s poses and $j$'s poses. 
In contrast, $h_i$ is formed by relative measurements within robot $i$'s own trajectory. 

Similar to the way a pose graph is defined, we can encode the structure of \eqref{eq:P} using a \emph{robot-level graph} $G_{\Rcal} \triangleq (\Rcal, E_{\Rcal})$. 
In $G_{\Rcal}$, two robots $i,j \in \Rcal$ are connected if they share any relative measurement $(i_{\tau}, j_s) \in E$ in the pose graph. 
In this case, we call $j$ a \emph{neighboring robot} of $i$, 
and $j_s$ a \emph{neighboring pose} of robot $i$.
Figure~\ref{fig:robot_graph} shows the robot-level graph corresponding to the pose graph in Figure~\ref{fig:pose_graph}.

In the literature, neighboring poses are also referred to as the \emph{separators} \cite{Choudhary2017Distributed}.
If a pose variable is not a neighboring pose to any other robots, we call this pose a \emph{private pose} \cite{Tian2019RBCD}.
We note that for robot $i$ to evaluate the shared cost $f_{ij}$, it only needs to know its neighboring poses in robot $j$'s trajectory (see Figure~\ref{fig:example_graph}). 
This property is crucial to preserve the \emph{privacy} of participating robots \cite{Choudhary2017Distributed,Tian2019RBCD}, i.e., at any time, robot does not need to share its private poses with any of its teammates. 





